LLM for Complex Reasoning Task: An Exploratory Study in Fermi Problems

Fermi Problems (FPs) are mathematical reasoning tasks that require human-like logic and numerical reasoning. Unlike other reasoning questions, FPs often involve real-world impracticalities or ambiguous concepts, making them challenging even for humans to solve. Despite advancements in AI, particularly with large language models (LLMs) in various reasoning tasks, FPs remain relatively under-explored. This work conducted an exploratory study to examine the capabilities and limitations of LLMs in solving FPs. We first evaluated the overall performance of three advanced LLMs using a publicly available FP dataset. We designed prompts according to the recently proposed TELeR taxonomy, including a zero-shot scenario. Results indicated that all three LLMs achieved a fp_score (range between 0 - 1) below 0.5, underscoring the inherent difficulty of these reasoning tasks. To further investigate, we categorized FPs into standard and specific questions, hypothesizing that LLMs would perform better on standard questions, which are characterized by clarity and conciseness, than on specific ones. Comparative experiments confirmed this hypothesis, demonstrating that LLMs performed better on standard FPs in terms of both accuracy and efficiency.

==> Tables/intersection_examples.tex <==


\begin{table*}[!ht]\small
\centering

% \ra{1.2}
% \adjustbox{max width=\textwidth}{%
% \begin{tabular}{C{3.5cm} | C{3.5cm} | C{3.5cm} | C{5.5cm}} %| m{0.8cm} | m{2cm}}
% \toprule
% \multicolumn{4}{c|}{\textbf{Narrative Pair Example \# 1}}\\
% \hline
% \multicolumn{2}{c|}{\textbf{Narrative 1:} $\mathbf{N_1}$} &
% \multicolumn{2}{c}{\textbf{Narrative 2:} $\mathbf{N_2}$} \\
% \hline
% \multicolumn{2}{C{8cm}|}{
% %% D1
% \hlgreen{
% WASHINGTON -- U.S. intelligence and law enforcement agencies have confirmed that President Donald Trump's campaign aides and associates had constant contact with Russian intelligence officials before the election, directly contradicting public statements made by top administration officials. 
% }
% On Jan. 15, shortly before Trump took office, Vice President Mike Pence repeatedly said on television that there were zero contacts between the campaign and Russian officials. 
% $\mathbf{\dotso}$

% \hlgreen{
% Pence also answered "of course not" when asked a similar question that day by "Fox News Sunday" host Chris Wallace
% $\mathbf{\dotso}$

% Trump himself also denied these interactions
% $\mathbf{\dotso}$

% }
% "There's nothing that would conclude me that anything different has changed with respect to that time period," Spicer said. 
% $\mathbf{\dotso}$

% %% -----------------------------------------
% } &
% \multicolumn{2}{C{8cm}}{
% %% -----------------------------------------
% %% D2
% \hlgreen{
% President Trump said Wednesday that new reports saying his associates had contact with Russian officials during last year's campaign are "non-sense"} and accused the U.S. intelligence community of illegally leaking information to news outlets. 
% \hlgreen{
% "This Russian connection non-sense} is merely an attempt to cover-up the many mistakes made in Hillary Clinton's losing campaign," Mr. Trump tweeted. 
% $\mathbf{\dotso}$

% Among those supposedly communicating with Russian nationals was former Trump campaign chairman Paul Manafort, the report said. 
% \hlgreen{Mr. Manafort denied that he ever knowingly talked to any intelligence official "or anyone}
% %% -----------------------------------------
% } \\
% \hline
% \multicolumn{4}{c}{\textbf{Reference Overlap Summaries}} \\\hline
%   \multicolumn{1}{c}{\textbf{A\textsubscript{1}}} &
%   \multicolumn{1}{c}{\textbf{A\textsubscript{2}}} &
%   \multicolumn{1}{c}{\textbf{A\textsubscript{3}}} &
%   \multicolumn{1}{c}{\textbf{AllSides}}
%   \\


% \hline
% %% A1
% President Trump and the Trump administration deny allegations that advisers close to Trump were in constant communication during the campaign with Russians known to US intelligence.
% &
% %% A2
% Trump denied climas that advisers close to him were in "constant communication during the campaign with Russians known to US intelligence.
% &
% %% A3
% Donald Trump and his group claimed that there is no contact with Russian officials during his last year's campaign. 
% &
% %% A4
% Russian intelligence officials made repeated contact with members of President Trump's campaign staff, according to new reports that cite anonymous U.S. officials. American agencies were concerned about the contacts but haven't seen proof of collusion between the campaign and the Russian security apparatus.
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \midrule
% \midrule


% \multicolumn{4}{c|}{\textbf{Narrative Pair Example \# 2}}\\\hline
% \multicolumn{2}{c|}{\textbf{Narrative 1:} $\mathbf{N_1}$} &
% \multicolumn{2}{c}{\textbf{Narrative 2:} $\mathbf{N_2}$} \\
% \hline

% \multicolumn{2}{C{8cm}|}{
% % %% -----------------------------------------
% %% D1
% John McCain is out of McConnell's clutches for a week or two. 
% \hlgreen{
% While Sen. John McCain remains in Arizona recovering from Friday's craniotomy, surgery to remove a 5 cm blood clot from above his left eye}, business will not go on as usual in Washington. 
% \hlgreen{
% Majority Leader Mitch McConnell, who has to have every Republican senator voting to have a prayer of passing Trumpcare, has postponed the vote for the week or two (more likely two) that McCain's recovery will take.
% }
% That means there's more time for opponents to fight this thing, from the side of all of us trying to keep 22 million people from losing insurance and from the other side. 
% $\mathbf{\dotso}$

% \hlgreen{With both Paul and Sen. Susan Collins (R-ME) solid "no" votes on the bill}, opponents only need one more out of the eight or so who've expressed reservations about the bill and the secretive, exclusive process McConnell
% %% -----------------------------------------
% } &
% \multicolumn{2}{C{8cm}}{
% %% -----------------------------------------
% %% D2
% \hlgreen{WASHINGTON - The Republican effort to repeal and replace Obamacare faces a major setback as Sen. John McCain, R-Ariz., left the nation's capital for surgery on his eye. 
% Over the weekend, Senate Majority Leader Mitch McConnell, R-Ky., announced the scheduled Better Care Act vote would be delayed indefinitely because of McCain's absence.}
% Subsequently, the Congressional Budget Office (CBO) also delayed its analysis of the bill. 
% \hlgreen{With two Republican senators opposed to the measure, McConnell needs as least 50 "yes" votes to pass it.}
% \hlgreen{Sen. Rand Paul, R-Ky., says the bill, which keeps taxes on investments and other pieces of Obamacare, doesn't go far enough. 
% Moderate Sen. Susan Collins, R-Maine, is also withholding her support because it would slow the rate of growth in spending on Medicaid.}
% $\mathbf{\dotso}$

% %% -----------------------------------------
% } \\
% \hline
% \multicolumn{4}{c}{\textbf{Reference Overlap Summaries}} \\\hline
% \multicolumn{1}{c}{\textbf{A\textsubscript{1}}} &
%   \multicolumn{1}{c}{\textbf{A\textsubscript{2}}} &
%   \multicolumn{1}{c}{\textbf{A\textsubscript{3}}} &
%   \multicolumn{1}{c}{\textbf{AllSides}}
%   \\


% \hline

% %% A1
% Sen. John McCain remains in Arizona recovering from eye surgery. Senate Majority Leader Mitch  McConnell postponed the vote due to McCain's absence. Two Republican senators opposed to the bill. Possibility of bill failing.
% &
% %% A2
% Sen. John McCain remains unavailable because of the surgery on his eye. Senate Majority Leader Mitch McConnell delayed the vote in his absence. Sen. Rand Paul and Sen. Susan Collins said "no" votes on the bill.
% &
% %% A3
% Senate Majority Leader Mitch McConnell, R-Ky., announced the scheduled health care vote would be delayed indefinitely because of McCain's absence.
% &
% %% A4
% Senate Majority Leader Mitch McConnell, R-Ky., announced the scheduled Better Care Act vote would be delayed indefinitely because of McCain's absence.
% \\
% \bottomrule
% \end{tabular}
% }
% \caption{Some examples of \textit{SOS} references from 3 human annotators (\textbf{A\textsubscript{i}}) and the AllSides ``theme-description'' for a given narrative pair $\{N_1, N_2\}$. 
% ($\mathbf{\dotso}$) denotes some sentences which for not shown for brevity. More examples can be found over \href{https://karmake2.github.io/publications/}{here}. Having multiple human annotators is critical to perform robust evaluation, but it is laborious and time-consuming on humans' part. This also shows that the lack of available datasets is a huge challenge for the SOS task. 
% }

% \begin{table}[h]
\centering
\small % 缩小字体
\begin{tabular}{|c|c|c|c|c|}
  \hline
  \multirow{2}{*}{Model Name} & \diagbox{Prompt Level}{Question Type} & Outlier & Uninformative Question & Informative Question \\
  \cline{2-5}
  % & Level &  &  &  \\
  \hline
  \multirow{3}{*}{GPT-turbo-3.5} & 0 & 26 & 2& 2\\
  \cline{2-5}
  & 2 & 18 & 8 & 4 \\
  \cline{2-5}
  & 4 & 25 & 3 & 2 \\
  \hline
  \multirow{3}{*}{GPT-turbo-4} & 0 & 21 & 4 & 5 \\
  \cline{2-5}
  & 2 & 19 & 5 & 6 \\
  \cline{2-5}
  & 4 & 16 & 7& 7 \\
  \hline
\end{tabular}

\caption{The number of question type of ChatGPT Model}

\vspace{1cm}
\label{table:qualitative_analysis}
\end{table*}

==> Tables/prompt_example.tex <==
% \documentclass{article}
% \usepackage{multirow}
% \usepackage{diagbox}
% \usepackage{caption}

\begin{table}[h]
\centering
\small % 缩小字体
\begin{tabular}{|c|c|c|c|c|}
  \hline
  \multirow{2}{*}{Model Name} & \diagbox{Prompt Level}{Question Type} & Outlier & Uninformative Question & Informative Question \\
  \cline{2-5}
  \hline
  \multirow{3}{*}{GPT-turbo-3.5} & 0 & 26 & 2& 2\\
  \cline{2-5}
  & 2 & 18 & 8 & 4 \\
  \cline{2-5}
  & 4 & 25 & 3 & 2 \\
  \hline
  \multirow{3}{*}{GPT-turbo-4} & 0 & 21 & 4 & 5 \\
  \cline{2-5}
  & 2 & 19 & 5 & 6 \\
  \cline{2-5}
  & 4 & 16 & 7& 7 \\
  \hline
\end{tabular}

\caption{The number of question type of ChatGPT Model}

\vspace{1cm}
\caption{ChatGPT and Bard has different understanding of conflicts in the two narratives}
\label{table:prompt_example}


\end{table}
